Classification-Based Opinion Formation Model Embedding Agents' Psychological Traits

We propose an agent-based opinion formation model characterised by a two-fold novelty. First, we realistically assume that each agent cannot measure the opinion of its neighbours with infinite resolution and accuracy, and hence it can only classify the opinion of others as agreeing much more, or more, or comparably, or less, or much less (than itself) with a given statement. This leads to a classification-based rule for opinion update. Second, we consider three complementary agent traits suggested by significant sociological and psychological research: conformism, radicalism and stubbornness. We rely on World Values Survey data to show that the proposed model has the potential to predict the evolution of opinions in real life: the classification-based approach and complementary agent traits produce rich collective behaviours, such as polarisation, consensus, and clustering, which can yield predicted opinions similar to survey results.

==> FriedkinJohnsenModel.tex <==
\begin{table}[h!]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{||c || c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c||} 
\hline\hline 
& C1 &  C2 &  C3 &  C4 &  C5 &  C6 &  C7 &  C8 &  C9 &  C10 &  C11 &  C12 &  C13 &  C14 &  C15 &  C16 &  C17 &  C18 &  C19 &  C20 &  C21 &  C22 &  C23 &  C24 &  C25 &  C26 \\ 
\hline\hline 
 Q1 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 8 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 6.2 &  \cellcolor{green!20} 2.6 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 1.4 &  \cellcolor{green!20} 4.8 &  \cellcolor{green!20} 5.4 &  \cellcolor{red!20} 9.4 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 2.6 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 10.6 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 5.6 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 5.4 \\ 
 Q2 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 1.4 &  \cellcolor{red!20} 8.8 &  \cellcolor{red!20} 7.4 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 14 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 13.8 &  \cellcolor{green!20} 2.4 &  \cellcolor{red!20} 8.6 &  \cellcolor{red!20} 9 &  \cellcolor{green!20} 1.4 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 6.4 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 3.8 \\ 
 Q3 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 6 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 2.2 &  \cellcolor{red!20} 7 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 13.4 &  \cellcolor{red!20} 11 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 4.8 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 10 &  \cellcolor{red!20} 18 &  \cellcolor{green!20} 2 &  \cellcolor{green!20} 1.4 &  \cellcolor{red!20} 9.4 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 1.4 &  \cellcolor{red!20} 9.4 &  \cellcolor{green!20} 2 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 5.4 &  \cellcolor{red!20} 8.6 \\ 
 Q4 &  \cellcolor{red!20} 15.6 &  \cellcolor{red!20} 12.2 &  \cellcolor{red!20} 18.6 &  \cellcolor{red!20} 19 &  \cellcolor{red!20} 29.4 &  \cellcolor{red!20} 9.8 &  \cellcolor{red!20} 10.8 &  \cellcolor{red!20} 25 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 15.6 &  \cellcolor{red!20} 9.6 &  \cellcolor{red!20} 9.8 &  \cellcolor{red!20} 10.8 &  \cellcolor{red!20} 24.4 &  \cellcolor{red!20} 17.8 &  \cellcolor{green!20} 5.6 &  \cellcolor{green!20} 6.2 &  \cellcolor{red!20} 17.2 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 38 &  \cellcolor{green!20} 2.4 &  \cellcolor{red!20} 15.8 &  \cellcolor{green!20} 5.4 &  \cellcolor{red!20} 52 &  \cellcolor{red!20} 14.2 &  \cellcolor{red!20} 8 \\ 
 Q5 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 6.6 &  \cellcolor{red!20} 8.4 &  \cellcolor{red!20} 13.2 &  \cellcolor{green!20} 4.6 &  \cellcolor{green!20} 4.8 &  \cellcolor{red!20} 8.2 &  \cellcolor{red!20} 10.4 &  \cellcolor{red!20} 18.4 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 9.2 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 7.6 &  \cellcolor{red!20} 23.6 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 11.2 &  \cellcolor{green!20} 0.8 &  \cellcolor{red!20} 8.8 &  \cellcolor{green!20} 0.4 &  \cellcolor{red!20} 12 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 5.6 &  \cellcolor{green!20} 6.6 &  \cellcolor{green!20} 5 \\ 
 Q6 &  \cellcolor{green!20} 5 &  \cellcolor{red!20} 7.8 &  \cellcolor{green!20} 6.4 &  \cellcolor{green!20} 5.8 &  \cellcolor{red!20} 13.8 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 14.6 &  \cellcolor{red!20} 7.6 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 8 &  \cellcolor{red!20} 11.8 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 10.2 &  \cellcolor{green!20} 3.6 &  \cellcolor{red!20} 13 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 14.8 &  \cellcolor{green!20} 0.4 &  \cellcolor{red!20} 23.8 &  \cellcolor{red!20} 11.8 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 15.8 &  \cellcolor{green!20} 4.6 &  \cellcolor{red!20} 7.4 \\ 
 Q7 &  \cellcolor{red!20} 7.2 &  \cellcolor{red!20} 7 &  \cellcolor{red!20} 11.6 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 4.8 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 8.4 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 11.8 &  \cellcolor{green!20} 5.4 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 11.8 &  \cellcolor{red!20} 7.8 &  \cellcolor{red!20} 25.2 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 6.2 &  \cellcolor{green!20} 0.6 &  \cellcolor{green!20} 6.8 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 8 \\ 
 Q8 &  \cellcolor{red!20} 10.6 &  \cellcolor{red!20} 8.6 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 11.2 &  \cellcolor{green!20} 5.4 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 5.2 &  \cellcolor{green!20} 4.6 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 12.6 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 9.2 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 21.8 &  \cellcolor{green!20} 5.2 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 5 &  \cellcolor{red!20} 14.2 &  \cellcolor{green!20} 0.4 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 8 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 4.6 \\ 
 Q9 &  \cellcolor{red!20} 13 &  \cellcolor{green!20} 6.6 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 2.2 &  \cellcolor{red!20} 20.6 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 9 &  \cellcolor{green!20} 6.6 &  \cellcolor{red!20} 13.4 &  \cellcolor{red!20} 15.2 &  \cellcolor{red!20} 11.2 &  \cellcolor{green!20} 3.6 &  \cellcolor{red!20} 15.4 &  \cellcolor{red!20} 8.8 &  \cellcolor{red!20} 8.4 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 7 &  \cellcolor{red!20} 15.6 &  \cellcolor{green!20} 6.6 &  \cellcolor{red!20} 10 &  \cellcolor{green!20} 5.6 &  \cellcolor{green!20} 4.2 &  \cellcolor{red!20} 9.8 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 6.6 &  \cellcolor{red!20} 14 \\ 
 Q10 &  \cellcolor{red!20} 17 &  \cellcolor{red!20} 9.8 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 20 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 8.4 &  \cellcolor{red!20} 11.8 &  \cellcolor{red!20} 11.8 &  \cellcolor{red!20} 10 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 9.2 &  \cellcolor{red!20} 7.4 &  \cellcolor{green!20} 6.8 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 5.4 &  \cellcolor{red!20} 11.2 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 9.4 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 10.8 &  \cellcolor{red!20} 8.6 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 18 \\ 
 Q11 &  \cellcolor{red!20} 18.2 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 6.2 &  \cellcolor{green!20} 2.8 &  \cellcolor{red!20} 12.8 &  \cellcolor{red!20} 9.6 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 10.4 &  \cellcolor{red!20} 12 &  \cellcolor{red!20} 13.6 &  \cellcolor{red!20} 10.4 &  \cellcolor{green!20} 1.2 &  \cellcolor{red!20} 19.8 &  \cellcolor{red!20} 10.2 &  \cellcolor{red!20} 17.6 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 14.2 &  \cellcolor{red!20} 12.2 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 8.4 &  \cellcolor{red!20} 13.8 &  \cellcolor{red!20} 17.4 &  \cellcolor{green!20} 5.8 &  \cellcolor{red!20} 7.4 &  \cellcolor{green!20} 4.6 &  \cellcolor{green!20} 3.8 \\ 
 Q12 &  \cellcolor{red!20} 13.4 &  \cellcolor{red!20} 9.6 &  \cellcolor{green!20} 6 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 31.8 &  \cellcolor{green!20} 6.4 &  \cellcolor{red!20} 11.6 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 19.8 &  \cellcolor{red!20} 16.2 &  \cellcolor{green!20} 6.4 &  \cellcolor{red!20} 13.8 &  \cellcolor{red!20} 9.6 &  \cellcolor{green!20} 4.8 &  \cellcolor{green!20} 0.6 &  \cellcolor{red!20} 8.6 &  \cellcolor{red!20} 9.2 &  \cellcolor{red!20} 11.6 &  \cellcolor{red!20} 8.4 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 32.2 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 13 \\ 
 Q13 &  \cellcolor{red!20} 13.8 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 6.8 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 1.4 &  \cellcolor{green!20} 1.2 &  \cellcolor{red!20} 8 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 15 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 12 &  \cellcolor{green!20} 3.4 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 17.4 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 4.8 &  \cellcolor{green!20} 2.2 &  \cellcolor{red!20} 64.8 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 6.2 &  \cellcolor{red!20} 9.6 \\ 
 Q14 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 7.4 &  \cellcolor{red!20} 7.4 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 6.8 &  \cellcolor{green!20} 0.2 &  \cellcolor{green!20} 6.4 &  \cellcolor{red!20} 8 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 23.6 &  \cellcolor{red!20} 7 &  \cellcolor{green!20} 6.4 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 35.2 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 5.4 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 25 &  \cellcolor{red!20} 12 &  \cellcolor{red!20} 10 &  \cellcolor{green!20} 2.8 &  \cellcolor{red!20} 10.2 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 5.4 \\ 
 Q15 &  \cellcolor{green!20} 2.8 &  \cellcolor{red!20} 18.4 &  \cellcolor{green!20} 2.6 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 0.8 &  \cellcolor{red!20} 12.2 &  \cellcolor{red!20} 17.4 &  \cellcolor{green!20} 0.6 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 17.6 &  \cellcolor{green!20} 6 &  \cellcolor{green!20} 0.4 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 7.6 &  \cellcolor{red!20} 26 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 0.8 &  \cellcolor{red!20} 17 &  \cellcolor{red!20} 8.4 &  \cellcolor{green!20} 2.6 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 8.6 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 3.4 \\ 
 Q16 &  \cellcolor{green!20} 0.6 &  \cellcolor{green!20} 4.8 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 2 &  \cellcolor{green!20} 0.4 &  \cellcolor{green!20} 5 &  \cellcolor{red!20} 14.2 &  \cellcolor{green!20} 5.6 &  \cellcolor{green!20} 0.6 &  \cellcolor{red!20} 15 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 2.6 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 35.4 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 0.4 &  \cellcolor{red!20} 16.4 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 0 &  \cellcolor{green!20} 4.6 &  \cellcolor{green!20} 0.6 &  \cellcolor{green!20} 4.8 \\ 
 Q17 &  \cellcolor{red!20} 13.8 &  \cellcolor{red!20} 10.2 &  \cellcolor{green!20} 5.8 &  \cellcolor{green!20} 6.6 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 17.6 &  \cellcolor{green!20} 2.2 &  \cellcolor{red!20} 7.6 &  \cellcolor{red!20} 9.2 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 8.6 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 7.8 &  \cellcolor{red!20} 22.4 &  \cellcolor{red!20} 7.4 &  \cellcolor{green!20} 3.4 &  \cellcolor{red!20} 9.2 &  \cellcolor{red!20} 10 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 10.6 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 14.4 &  \cellcolor{red!20} 12.6 \\ 
 Q18 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 16.2 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 10 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 21.2 &  \cellcolor{red!20} 10.4 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 14 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 4.8 &  \cellcolor{red!20} 11.8 &  \cellcolor{red!20} 22.4 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 6.4 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 8.8 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 5.6 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 11.2 \\ 
 Q19 &  \cellcolor{green!20} 4.6 &  \cellcolor{red!20} 14.4 &  \cellcolor{red!20} 9.2 &  \cellcolor{red!20} 16.8 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 26.6 &  \cellcolor{red!20} 13.8 &  \cellcolor{green!20} 4.6 &  \cellcolor{red!20} 11.6 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 5.2 &  \cellcolor{green!20} 6.6 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 9 &  \cellcolor{green!20} 6.4 &  \cellcolor{green!20} 4.6 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 14.4 &  \cellcolor{red!20} 7 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 2.8 &  \cellcolor{red!20} 7.2 &  \cellcolor{red!20} 7.4 \\ 
 Q20 &  \cellcolor{green!20} 5.4 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 4.6 &  \cellcolor{red!20} 10.8 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 4.8 &  \cellcolor{red!20} 20.6 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 8.6 &  \cellcolor{red!20} 12.2 &  \cellcolor{green!20} 3.6 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 5 &  \cellcolor{red!20} 32.2 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 5.2 &  \cellcolor{green!20} 6.6 &  \cellcolor{red!20} 9.4 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 5.8 &  \cellcolor{red!20} 10 \\ 
 Q21 &  \cellcolor{green!20} 1.4 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 0 &  \cellcolor{red!20} 9 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 0 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 15.6 &  \cellcolor{green!20} 0.8 &  \cellcolor{green!20} 4.2 &  \cellcolor{red!20} 11 &  \cellcolor{green!20} 2.6 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 1.4 &  \cellcolor{red!20} 28.2 &  \cellcolor{green!20} 0.6 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 0.2 &  \cellcolor{red!20} 12.4 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 0.8 &  \cellcolor{green!20} 0.6 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 4.6 \\ 
 Q22 &  \cellcolor{green!20} 4.2 &  \cellcolor{red!20} 9.2 &  \cellcolor{red!20} 8.6 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 7.2 &  \cellcolor{red!20} 11 &  \cellcolor{red!20} 19.2 &  \cellcolor{red!20} 11.8 &  \cellcolor{red!20} 13.8 &  \cellcolor{green!20} 4.8 &  \cellcolor{red!20} 10.8 &  \cellcolor{green!20} 5.2 &  \cellcolor{red!20} 10.6 &  \cellcolor{red!20} 12.2 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 0.6 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 2.6 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 24.6 &  \cellcolor{red!20} 26.6 &  \cellcolor{red!20} 10 &  \cellcolor{green!20} 4.4 &  \cellcolor{red!20} 7.8 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 8 \\ 
 Q23 &  \cellcolor{green!20} 5.6 &  \cellcolor{red!20} 10.2 &  \cellcolor{red!20} 7.2 &  \cellcolor{red!20} 13 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 14.2 &  \cellcolor{green!20} 3.4 &  \cellcolor{green!20} 6.2 &  \cellcolor{red!20} 18.6 &  \cellcolor{red!20} 11.8 &  \cellcolor{red!20} 16 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 5.8 &  \cellcolor{red!20} 15.8 &  \cellcolor{green!20} 5 &  \cellcolor{red!20} 11.4 &  \cellcolor{green!20} 5 &  \cellcolor{red!20} 8.6 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 18.6 &  \cellcolor{red!20} 13.6 &  \cellcolor{green!20} 6.2 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 3.4 \\ 
 Q24 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 5.8 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 17.8 &  \cellcolor{green!20} 2.4 &  \cellcolor{red!20} 12.8 &  \cellcolor{green!20} 2.2 &  \cellcolor{red!20} 12 &  \cellcolor{red!20} 20.6 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 13.2 &  \cellcolor{green!20} 5 &  \cellcolor{green!20} 3.2 &  \cellcolor{red!20} 17.2 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 15.4 &  \cellcolor{green!20} 0.8 &  \cellcolor{green!20} 5.2 &  \cellcolor{green!20} 4.2 &  \cellcolor{red!20} 17.6 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 4.6 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 3.2 \\ 
 Q25 &  \cellcolor{green!20} 4.8 &  \cellcolor{red!20} 8.8 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 1.8 &  \cellcolor{green!20} 5.6 &  \cellcolor{red!20} 20.2 &  \cellcolor{red!20} 16.4 &  \cellcolor{red!20} 10.6 &  \cellcolor{red!20} 8 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 12.4 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 16.6 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 18.4 &  \cellcolor{green!20} 1.4 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 0.8 &  \cellcolor{red!20} 19.2 &  \cellcolor{red!20} 13 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 3.4 &  \cellcolor{green!20} 4.6 &  \cellcolor{green!20} 3.4 &  \cellcolor{green!20} 3 \\ 
 Q26 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 14.8 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 25.2 &  \cellcolor{green!20} 4 &  \cellcolor{red!20} 11.8 &  \cellcolor{green!20} 5.2 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 3.2 &  \cellcolor{green!20} 1.6 &  \cellcolor{red!20} 17.6 &  \cellcolor{green!20} 0.8 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 2.6 &  \cellcolor{red!20} 17.4 &  \cellcolor{red!20} 18.8 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 7.4 &  \cellcolor{red!20} 10 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 2.4 \\ 
 Q27 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 9 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 6.2 &  \cellcolor{red!20} 16.6 &  \cellcolor{red!20} 35.2 &  \cellcolor{red!20} 23.4 &  \cellcolor{red!20} 8.4 &  \cellcolor{red!20} 26.2 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 20.8 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 15.8 &  \cellcolor{green!20} 0.6 &  \cellcolor{red!20} 12.6 &  \cellcolor{green!20} 1.4 &  \cellcolor{red!20} 14 &  \cellcolor{green!20} 5.4 &  \cellcolor{red!20} 19 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 6.4 &  \cellcolor{red!20} 12.6 &  \cellcolor{green!20} 2.8 &  \cellcolor{green!20} 6.2 &  \cellcolor{red!20} 8.2 \\ 
 Q28 &  \cellcolor{green!20} 4.4 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 0.4 &  \cellcolor{green!20} 6.2 &  \cellcolor{red!20} 9.2 &  \cellcolor{red!20} 19.6 &  \cellcolor{red!20} 9.2 &  \cellcolor{green!20} 3.8 &  \cellcolor{red!20} 15.2 &  \cellcolor{red!20} 8.4 &  \cellcolor{red!20} 17.4 &  \cellcolor{green!20} 1.4 &  \cellcolor{green!20} 4.2 &  \cellcolor{red!20} 10.8 &  \cellcolor{green!20} 1.8 &  \cellcolor{red!20} 14.2 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 4.8 &  \cellcolor{red!20} 9.4 &  \cellcolor{red!20} 10.4 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 6.4 &  \cellcolor{red!20} 8.2 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 2.2 &  \cellcolor{green!20} 4 \\ 
 Q29 &  \cellcolor{green!20} 1 &  \cellcolor{red!20} 8 &  \cellcolor{green!20} 4.2 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 1.2 &  \cellcolor{green!20} 6 &  \cellcolor{red!20} 9.8 &  \cellcolor{red!20} 7.6 &  \cellcolor{red!20} 16.4 &  \cellcolor{green!20} 4.8 &  \cellcolor{red!20} 12.6 &  \cellcolor{green!20} 3 &  \cellcolor{green!20} 1.4 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 2 &  \cellcolor{red!20} 17.6 &  \cellcolor{green!20} 0.2 &  \cellcolor{green!20} 4 &  \cellcolor{green!20} 1.4 &  \cellcolor{red!20} 9.4 &  \cellcolor{green!20} 0.8 &  \cellcolor{green!20} 2.4 &  \cellcolor{red!20} 9.6 &  \cellcolor{green!20} 2.4 &  \cellcolor{green!20} 1 &  \cellcolor{green!20} 0.4 \\ 
 Q30 &  \cellcolor{green!20} 2.2 &  \cellcolor{red!20} 10.4 &  \cellcolor{red!20} 11.8 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 21 &  \cellcolor{red!20} 7.4 &  \cellcolor{red!20} 20 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 16.6 &  \cellcolor{red!20} 7.2 &  \cellcolor{green!20} 3.4 &  \cellcolor{green!20} 5.8 &  \cellcolor{green!20} 3.4 &  \cellcolor{red!20} 18 &  \cellcolor{red!20} 20.6 &  \cellcolor{red!20} 8 &  \cellcolor{red!20} 11.2 &  \cellcolor{green!20} 3 &  \cellcolor{red!20} 8.4 &  \cellcolor{red!20} 9.4 &  \cellcolor{red!20} 7.8 &  \cellcolor{green!20} 1.6 &  \cellcolor{green!20} 6.8 &  \cellcolor{green!20} 3.8 &  \cellcolor{green!20} 0.8 &  \cellcolor{green!20} 1.8 \\ 
\hline 
Average & 6.4 & 7.5 & 5.5 & 6.5 & 7.8 & 7.8 & 7.1 & 11.6 & 10.4 & 6.5 & 11.9 & 4.1 & 5.9 & 9.9 & 6 & 15.1 & 4.4 & 6.4 & 3.3 & 16 & 6.4 & 5.1 & 4.2 & 8 & 4.4 & 6.8 \\ 
\hline 
Total & 190.6 & 224.8 & 165.2 & 194.8 & 232.6 & 232.8 & 212 & 347.4 & 311.6 & 193.8 & 357.8 & 124.2 & 176.4 & 297 & 179 & 452.2 & 133.4 & 192.8 & 99.8 & 480.6 & 191 & 152.2 & 126.8 & 238.8 & 131.4 & 203 \\ 
\hline\hline 
\end{tabular}}
\caption{Results of of the optimization problem using the Friedkin-Johnsen model.  From 780 possible question-country pairs 460 have a cost less than 7 (an accuracy of $59\%$ in total). The average cost of accepted question-country pairs is 3.3. }
\label{Tab:ResultsFJ}
\end{table} 

